Learning Part Motion of Articulated Objects Using Spatially Continuous Neural Implicit Representations

Articulated objects (e.g., doors and drawers) exist everywhere in our life. Different from rigid objects, articulated objects have higher degrees of freedom and are rich in geometries, semantics, and part functions. Modeling different kinds of parts and articulations with nerual networks plays an essential role in articulated object understanding and manipulation, and will further benefit 3D vision and robotics communities. To model articulated objects, most previous works directly encode articulated objects into feature representations, without specific designs for parts, articulations and part motions. In this paper, we introduce a novel framework that explicitly disentangles the part motion of articulated objects by predicting the transformation matrix of points on the part surface, using spatially continuous neural implicit representations to model the part motion smoothly in the space. More importantly, while many methods could only model a certain kind of joint motion (such as the revolution in the clockwise order), our proposed framework is generic to different kinds of joint motions in that transformation matrix can model diverse kinds of joint motions in the space. Quantitative and qualitative results of experiments over diverse categories of articulated objects demonstrate the effectiveness of our proposed framework.

==> tabs/CD_PAE.tex <==
\begin{tabularx}{30.12cm}{@{}l>{\centering\arraybackslash}m{0.95cm}>{\centering\arraybackslash}m{0.95cm}>{\centering\arraybackslash}m{0.95cm}>{\centering\arraybackslash}m{0.95cm}@{}}
    \toprule
    Method   & Oven-Refri & Refri-Oven & Door-Laptop & \\ \midrule
    \midrule
    A-SDF    & 37.7618 & 2.0164 & 2.2532 & \\ \midrule
    Ditto    & 3.9443 & 2.1832 & 2.3997 & \\ \midrule
    Ours w/o NIR & 15.5203 & 1.6832 & 2.3547 & \\ \midrule
    Ours & \textbf{2.5794} & \textbf{1.5440} & \textbf{2.0873} &   \\ \bottomrule
    \end{tabularx}

==> tabs/extrapolation.tex <==
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.95cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}@{}}
    \toprule
    Method   & Fridge & Oven & Door & Table &\\ \midrule \midrule
    \small{A-SDF}    & 4.2671 & 2.5514 & 5.3937 & 8.0931 & \\ \midrule
    Ditto    & 3.1738 & 1.9405 & 4.4676 & 8.5025 & \\ \midrule
    Ours     & \textbf{2.8376} & \textbf{1.7669} & \textbf{3.5298} & \textbf{7.0804} &  \\ \bottomrule
    \end{tabular}

==> tabs/interpolation.tex <==
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.95cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}>{\centering\arraybackslash}m{0.9cm}@{}}
    \toprule
    Method   & Fridge & Oven & Door & Table &\\ \midrule \midrule
    \small{A-SDF}    & 4.1248 & 1.6185 & 2.8883 & 8.3870 & \\ \midrule
    Ditto    & 3.2421 & 1.2861 & 2.5974 & 9.8180 & \\ \midrule
    Ours     & \textbf{2.1256} & \textbf{1.2364} & \textbf{2.1330} & \textbf{8.1688} &  \\ \bottomrule
    \end{tabular}

==> tabs/multi_cat.tex <==
\begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    Setting   & Revolute-only & All-cat & \\ \midrule \midrule
    A-SDF    & 2.4125 & 2.1318 & \\ \midrule
    Ditto    & 2.5901 & 2.8800 & \\ \midrule
    Ours w/o NIR & 3.0751 & 10.7618 & \\ \midrule
    Ours & \textbf{2.3945} & \textbf{2.1042} & \\ \bottomrule
    \end{tabular}

==> tabs/multi_cat_data.tex <==
\begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    Category   & Laptop & Door & Refrigerator & Oven & Microwave & Stapler & Table & \\ \midrule \midrule 
    Number of instances    & 600 & 1200 & 1000 & 400 & 400 & 400 & 400 & \\ \bottomrule
    \end{tabular}

==> tabs/multi_cat_on_table.tex <==
\begin{tabular}{@{}lcccccccccc@{}}
    \toprule
    Setting   & Before tune & After tune & \\ \midrule \midrule 
    A-SDF    & 11.3914 & 2.7786 & \\ \midrule
    Ditto    & 12.3114 & 3.3318 & \\ \midrule
    Ours w/o NIR & 11.2056 & 14.9411 & \\ \midrule
    Ours & \textbf{10.7623} & \textbf{2.4877} & \\ \bottomrule
    \end{tabular}

==> tex/5_Experiment.tex <==
\section{Experiments}
\label{sec:experiment}


We conduct our experiments using the large-scale PartNet-Mobility~\cite{chang2015shapenet, Mo_2019_CVPR, Xiang_2020_SAPIEN} dataset of 3D articulated objects, covering over 7 object categories. We evaluate the performance of our method in several tasks including: 1) the articulated object generation for unseen objects in training categories, 
2) few-shot articulated object generation for novel object categories, % after a short period of finetuning, 
and 3) the interpolation and extrapolation of the spatial continuous NIR. %in the latent representation space.
Quantitative and qualitative results compared to several baselines and an ablated version, demonstrating our method's superiority over other methods. 

\subsection{Experiment Settings and Datasets}

% \subsubsection{Tasks}

% \textbf{Experiment Settings.} 
% \yan{this paragraph is optional, may explain some implementation details, e.g. training/inference settings, }
% \textbf{Datasets.}
We conduct our experiments on the large-scale PartNet-Mobility dataset~\cite{chang2015shapenet, Mo_2019_CVPR, Xiang_2020_SAPIEN}, %PartNet-Mobility is a large dataset of
containing
diverse 3D articulated objects. % with 2,346 CAD models from 46 object categories. 
% Compared to the Shape2Motion Dataset~\cite{wang2019shape2motion} used by A-SDF~\cite{mu2021sdf} and Ditto~\cite{jiang2022ditto}, PartNet-Mobility dataset owns more diverse motion parts and articulations within an object category, making it more challenging to learn the articulated object generation.
In our experiments, we select 7 categories from the PartNet-Mobility dataset, which are laptop, stapler, door, scissors, oven, refrigerator, microwave, table, and storage furniture.
To have a fair comparison, following the training settings of A-SDF~\cite{mu2021sdf}, we train a specific model for each object category.

\begin{figure*}[t]
    \centering  % left bottom right top)
    \includegraphics[trim={55, 20, 160, 0}, clip, scale=0.45]{figs/single_cat.pdf}
    \vspace{6mm}
    \caption{
    \textbf{Visualisation of generated objects in training categories} shows our method reserves the most detailed geometries of both articulated parts and object bases.
    For example, our model predicts the straightest door frame and the smoothest microwave door surface.
    % our method predicts the door frame straightly and the microwave door surface smoothly. %, but A-SDF and Ditto fail to predict them precisely.
    }
    \vspace{-2mm}
    \label{fig:single_cat}
\end{figure*}

\begin{table*}[htbp]
  \centering
  % \setlength{\tabcolsep}{1.2mm}
  \resizebox{\textwidth}{!}{
    \input{tabs/generation.tex}
    }
  \vspace{4mm}
  \caption{\textbf{Earth Mover’s Distance (EMD) on object generation in training categories.} %The quantitative results demonstrate that our proposed framework outperforms all other baselines and the ablated version in all training categories.
  }
  \label{tab_quan_train}
  \vspace{-2mm}
\end{table*}


\subsection{Baselines and Metrics}

We evaluate and compare our approach with the following two baselines and one ablation:

% \vspace{0.5mm}
\textbf{A-SDF}~\cite{mu2021sdf} represent objects with a shape code and an articulation code respectively. Given an articulated object shape, it first infers the shape and articulation codes, and then generates the shape at unseen angles by remaining the shape code unchanged and changing the articulation code.

% \vspace{0.5mm}
\textbf{Ditto}~\cite{jiang2022ditto} also takes two point clouds as input to learn the structure of an articulated object. Different from our method, it directly predicts the occupancy, the segmentation and the joint configuration to build a digital twin. The original paper demonstrates the point cloud reconstruct ablity, we modify it to take a new part pose as input and then generates the object with the new part pose.

% \yian{these two baselines all generate a mesh rather than a point cloud. shouldn't we declare how we transform the mesh to the point cloud? and how we use ditto to generate the point cloud in the new part pose?}
% directly decodes the point cloud and the joint configuration of an articulated object, and thus could build the digital twin.
% builds digital twins of articulated objects by jointly reconstructing the part-level geometry and articulation model in an explicit way.
% jointly infers object's part-level geometry and articulation model from the visual observations before and after an interaction. \yan{may add some difference in framework design(optional), if there is any modification, point out it}

% \vspace{0.5mm}
\textbf{Ours w/o NIR} is an ablated version of our method that directly predicts the transformation matrix for each point to generate the new point cloud without applying spatially continuous NIR as a middle step. We conduct this ablation version to demonstrate the effectiveness of our design using Spatial Transformation Feature Grid $G$.

% \paragraph{Metrics.}
To evaluate the generated objects and their similarity with the ground-truth objects, we apply the Earth Mover's Distance (EMD)~\cite{rubner2000earth} as the evaluation metric.
% EMD is utilized to estimate the distance between two distributions, we can calculate the EMD between two point clouds by calculating the minimum amount of point movements needed to change the generated object point cloud into the target.


% \begin{figure}[t]
%     \centering % left bottom right top)
%     \includegraphics[trim={260, 5, 260, 0}, clip, scale=0.58]{figs/finetune.pdf}
%     \caption{
%     \textbf{Visualization of the generated articulated object (in novel categories)} shows that our method not only generates objects with the most accurate poses, but also reserves the most detailed geometries of both articulated parts and object bases.
%     }
%     \label{fig:finetune}
% \end{figure}

% \subsection{Articulated Object (in training category) Generation.} 
\subsection{Evaluation on Unseen Objects in Training Categories}
In this task, given an articulated object in the training category with two point clouds and the corresponding part poses, we generate its point cloud with novel part poses. 

The quantitative results in Table~\ref{tab_quan_train} demonstrate that our proposed framework outperforms all other methods in all training categories with the lower EMD, which means that our generated articulated objects are the closest to the ground-truth shapes. The qualitative results in Figure~\ref{fig:single_cat} also show that our generated objects reserve the most detailed geometry of both the articulated part and the static base. In comparison, the performance of both Ditto and A-SDF is worse, for example, they both fail to predict the door frame straightly, and fail to predict the microwave door surface smoothly. 

The main reason behind this difference is, A-SDF and Ditto directly decode the whole point cloud into latent space, while our method takes the integrity of parts into consideration by querying the motion of each point in the original point cloud. This design best preserves the geometric features of the original shape because it is a one-to-one mapping from the original shape to the generated shape.

\begin{wraptable}{l}{6.5cm}
  \centering
  \vspace{-3mm}
  % \setlength{\tabcolsep}{1.2mm}
    \input{tabs/finetune.tex}
  \vspace{4mm}
  \caption{\textbf{Earth Mover’s Distance (EMD) on articulated object generation (in novel categories).} The results demonstrate that, after a short period of finetuning, our framework outperforms all other baselines and the ablated version in all novel categories.
  % \textbf{Quantitative results on finetune} \yan{xxx}
  }
  % \vspace{-1mm}
  \label{tab_quan_novel}
\end{wraptable}


\subsection{Evaluation on Novel Categories} 

In this task, we use the pretrained model in one category and finetune the model in a novel category using only a few objects in the novel category for a few epochs. Specifically, we use 8 objects in the novel category, and the finetuning time is one-twentieth of the training time from scratch.
% finetune the model for 2 hours, while it takes 40 hours to train a model from scratch. 
It is worth mentioning that the directions of the articulated part axes in the training set and finetuning set are different in these experiments (\emph{i.e.,} we train on the up-down opening ovens and finetune on the left-right opening refrigerators.)
% up-down opening or left-right opening).
This task aims to demonstrate that learning the part motions of articulated objects makes the model easier to adjust a novel kind of articulated object, as part motion is the shared property of all articulated objects. 
% \ruihai{xxx}


The quantitative results in Table~\ref{tab_quan_novel} show that our method achieves significantly better results with the lower EMD compared to all the baselines and the ablated version, especially in the Oven-Refrigerator block. The visualisation results of Figure~\ref{fig:finetune} also present that the generated objects of our method have the most accurate part poses and the most precise part geometry after a short-period finetuning. 
In comparison, A-SDF completely fails to predict the novel refrigerator after finetuning for a few epochs, which means that the representations learned by A-SDF are limited to the trained articulated object category and are hard to adjust to novel articulated shapes and joint configurations. 

\begin{wrapfigure}{r}{6cm}
    \centering % left bottom right top)
    \vspace{-0.6cm}
    \includegraphics[trim={260, 10, 300, 42}, clip, scale=0.42]{figs/finetune.pdf}
    \vspace{0.5mm}
    \caption{
    \textbf{Visualisation of the generated object in novel categories} shows our method maintains the geometries consistency with the origial object. 
    %not only generates objects with the most accurate poses, but also reserves the most detailed geometries of both articulated parts and object bases.
    }
    \vspace{-1.2cm}
    \label{fig:finetune}
\end{wrapfigure}

Our superior performance in novel categories against Ditto mainly comes from that we use the transformation matrix to represent part motion. Intuitively, a transformation matrix could represent any kind of motion in 3D space and is spatial continuous for points on the motion part. As a result, it has the potential to few-shot generalise to any kind of part motion no matter it is an up-down or a left-right opening door.


\subsection{Ablation Studies and Analysis}

We compare our method with the ablated version without Neural Implicit Representations (\textbf{Ours w/o NIR}). Results in Table~\ref{tab_quan_train} and Table~\ref{tab_quan_novel} show that NIR helps the generated point cloud to be closer to the ground-truth target, representing by the lower EMD between the generated objects and the ground-truth objects. 
From the visualisation in Figure~\ref{fig:single_cat} and Figure~\ref{fig:finetune}, we can observe that the point clouds generated with NIR have more accurate part pose and smoother part surface. Those results demonstrate that by using Spatially Continuous Neural Implicit Representation to model the part motion, our framework gets a better distribution for motion representations in the 3D space.

% \begin{figure}[t]
% \centering
% \begin{minipage}[t]{0.45\linewidth}
%     \centering % left bottom right top)
%     \includegraphics[trim={300, 460, 300, 65}, clip, scale=0.45]{figs/NIR_visual.pdf}
%     \vspace{0.4cm}
%     \caption{
%     \textbf{Visualization of the transformation on grid points.} We uniformly sampled points in the space as queries to the transformation grid, and represent the transformation direction by arrows. The results show the spatial distribution of the implicit representation. 
%     Note that in the second column, we represent the refrigerator in the top-down view, and represent the oven in the side view for better understanding.
%     % Details are shown in section \ref{sec:tranformation}.
%     }
%     \label{fig:NIR}
% \end{minipage}
% \hspace{0.05\linewidth}
% \begin{minipage}[t]{0.45\linewidth}
%     \centering % left bottom right top)
%     \includegraphics[trim={225, 65, 220, 20}, clip, scale=0.3]{figs/inter_extra.pdf}
%     \vspace{0.5cm}
%     \caption{
%     \textbf{Visualisation of the Interpolation and Extrapolation.} The lower and upper bound of interpolation or extrapolation are shown in light green and deep green, while our predictions are shown in medium green.
%     }
%     \label{fig:interpolation}
% \end{minipage}
% \end{figure}

\vspace{-0.3cm}

\subsection{Analysis of Transformation on Grid Points}
\label{sec:tranformation}
Figure~\ref{fig:inter_NIR} visualises the transformation grid of a refrigerator instance (in the first row) and an oven instance (in the second row). 
The figures on the left are displayed in 3D while the right ones are displayed in 2D. Note that for better visualisation and understanding, on the right, we represent the refrigerator in the top-down view, and represent the oven in the side view. 
The arrows forging circles centreing the ground-truth joint show that our model successfully projects the part motion to euclidean space. 
% Note that the 2D visualizations of the two objects are displayed in different directions to show the motion explicitly.

\subsection{Interpolation and Extrapolation} 

\begin{figure*}[t]
    \centering  % left bottom right top)
    \includegraphics[trim={550, 440, 550, 350}, clip, scale=0.45]{figs/inter_NIR.pdf}
    \vspace{4mm}
    \caption{
    \textbf{Visualisation of the transformation on grid points (left), and results of interpolation and extrapolation (right).}
    % The figure on the left shows \textbf{Visualization of the transformation on grid points.} We uniformly sampled points in the space as queries to the transformation grid, and represent the transformation direction by arrows. The results show the spatial distribution of the implicit representation. 
    % Note that in the second column, we represent the refrigerator in the top-down view, and represent the oven in the side view for better understanding.
    % The figure on the right shows \textbf{Visualisation of the Interpolation and Extrapolation.} The lower and upper bounds of interpolation or extrapolation are shown in light green and deep green, while our predictions are shown in medium green.
    }
    \vspace{-6mm}
    \label{fig:inter_NIR}
\end{figure*}

Interpolation and extrapolation between shapes is an essential ability for 3D object representations, in that it reveals the articulation part poses distribute continuously and densely in the representation. 
In this task, given two shapes of the same object, we generate the object with novel articulation degrees in between or beyond. 
% The ability to interpolate and extrapolate between shapes is essential for good 3D articulated object representations, for the reason that it reveals the dense articulation part poses distributing continuously and densely in the representation.
In Table~\ref{tab_inter_extrapolation}, quantitative results show that our method outperforms A-SDF and Ditto in both interpolation and extrapolation tasks.
% can reliably interpolate and extrapolate shapes. 
In Figure~\ref{fig:inter_NIR}, we represent the input parts with dark green and light green, and represent the generated part with medium green. We can observe that our method can reliably generate shapes, demonstrating that our representation of part motion is continuous and dense.
\vspace{-5mm}

% The ability to interpolate and extrapolate between shapes is important for a good 3D articulated object representation. First, as the articulation space is continuous, training models to densely cover all angles is infeasible. Second, training models with densely sampled angles takes huge amount of training time, which makes it hard for real-world applications. 
% In this section, given two articulated shapes of the same instance, we ask the models to output shapes with articulations in between or beyond.

% \subsection{Quantitative Results and Analysis}

% From Table~\ref{tab_quan}, Table~\ref{xxx} and Table~\ref{xxx}, it is clear that our proposed framework outperforms other methods in the quantitative metric.


% \subsection{Qualitative Results and Analysis}
% Figure~\ref{fig:single_cat} visualizes the generated articulated objects from the training categories, we can see that our method reserves the most detailed geometry of both the articulated part and the static base. Figure~\ref{fig:finetune} visualizes the generated objects from the novel categories after finetuning the model for a few epochs. We can find that the generated objects of our method have the most accurate poses and the most precise part geometry. In comparison, 

\begin{table}[t]
  \centering
  \vspace{4mm}
  % \setlength{\tabcolsep}{1.2mm}
    % \resizebox{\columnwidth}{!}{
    \input{tabs/inter_extra.tex}
    % }
  \vspace{4mm}
  \caption{
    \textbf{EMD on interpolation (Left) and extrapolation (Right) results.}
    }
  \label{tab_inter_extrapolation}
  \vspace{-5mm}
\end{table}

% \begin{table}[t]
% \begin{minipage}{.5\textwidth}
%   \centering
%   \vspace{1mm}
%     \input{tabs/interpolation.tex}
%   \vspace{3mm}
%   \caption{
%     \textbf{EMD on interpolation results.}
%   }
%   \vspace{-5mm}
%   \label{tab_interpolation}
% \end{minipage}\hfill
% \begin{minipage}{.5\textwidth}
%   \centering
%   \vspace{1mm}
%     \input{tabs/extrapolation.tex}
%   \vspace{3mm}
%   \caption{
%     \textbf{EMD on extrapolation results.}
%   }
%   \vspace{-5mm}
%   \label{tab_extrapolation}
% \end{minipage}
% \end{table}



% \floatsetup[table]{capposition=top}
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \begin{wraptable}{l}{3cm}
%   \centering
%   % \setlength{\tabcolsep}{1.3mm}
%   \vspace{1mm}
%   % \resizebox{\columnwidth}{!}{
%     \input{tabs/interpolation.tex}
%     % }
%   \vspace{2mm}
%   \caption{
%     \textbf{EMD on interpolation results.}
%   }
%   \label{tab_interpolation}
%   \vspace{2mm}
% \end{wraptable}

% \begin{wraptable}{r}{3cm}
%   \centering
%   % \setlength{\tabcolsep}{1.2mm}
%     % \resizebox{\columnwidth}{!}{
%     \input{tabs/extrapolation.tex}
%     % }
%   \vspace{2mm}
%   \caption{
%     \textbf{EMD on extrapolation results.}
%     }
%   \label{tab_extrapolation}
%   \vspace{2mm}
% \end{wraptable}

% \begin{multicols}{2}
% \begin{table}[t]
%   \centering
%   % \setlength{\tabcolsep}{1.3mm}
%   \vspace{1mm}
%   % \resizebox{\columnwidth}{!}{
%     \input{tabs/interpolation.tex}
%     % }
%   \vspace{2mm}
%   \caption{
%     \textbf{EMD on interpolation results.}
%   }
%   \label{tab_interpolation}
%   \vspace{2mm}
% \end{table}

% \begin{table}[t]
%   \centering
%   % \setlength{\tabcolsep}{1.2mm}
%     % \resizebox{\columnwidth}{!}{
%     \input{tabs/extrapolation.tex}
%     % }
%   \vspace{2mm}
%   \caption{
%     \textbf{EMD on extrapolation results.}
%     }
%   \label{tab_extrapolation}
%   \vspace{2mm}
% \end{table}
% \end{multicols}



==> tex/6_Conclusion.tex <==
\vspace{4mm}
\section{Conclusion}
\label{sec:conclusion}

In this paper, %to modelling and generating articulated objects, 
we propose a novel framework for modelling and generating articulated objects. %to learn part motions for articulated objects. 
To model the continuous articulations and motions smoothly, we adopt neural implicit representations (NIR) to predict the transformations of moving part points of the object. Experiments on different representative tasks %, including articulated object generation with novel poses in both training and novel categories, interpolation) 
demonstrate that our proposed framework outperforms other methods both quantitatively and qualitatively.
% \vspace{3mm}
% \textbf{Limitations and future work.} %Our framework learns from two point clouds of the same object, in the future, 
In this study, each object in the training set provides two point cloud under different part poses.
In the future, providing additional point clouds of an object under different part poses can help to understand articulated objects that have multiple joints. %and kinematics.
% taking more point clouds may help in % of different joints in a certain object.
% Besides, our work mainly focuses on the articulated object generation using the spatially continuous neural implicit representations, 

% \begin{wrapfigure}{r}{6cm}
%     \centering % left bottom right top)
%     \includegraphics[trim={0, 0, 0, 0}, clip, scale=0.3]{images/multi.pdf}
%     \vspace{2mm}
%     \caption{
%     \textbf{Generated multi-part cabinets with different part poses.}
%     }
%     \label{fig:multi_part}
% \end{wrapfigure}
